Does The Cloud Need Stabilizing?

The last decade has witnessed rapid proliferation of cloud computing. While even the smallest distributed programs (with 3-5 actions) produce many unanticipated error cases due to concurrency involved, it seems short of a miracle these web-services are able to operate at those vast scales. In this paper, we explore the factors that contribute most to the high-availability of cloud computing services and examine where self-stabilization could fit in that picture.

==> discuss2.tex <==
{\bf Does arbitrary state corruption occur in the clouds? Do we see state un-synchronization?}

+ For metadata, use ZK as coordination service and guard it well. But a corrupted/confused worker can write bad data to ZK, corrupting/confusing state as well. So guard those writes carefully, check ZK state before writing, check ZK state for invariant violations. ZK-side wrapper, enabled via Retroscope may help!
+ Nodes/Services are loosely coupled. But what about excessive fanout: problems may occur when some nodes don't respond. Could that lead to state un-syncronization?
+ What if a node fails not via a crash, but via returning incorrect answers? Is that a very bad thing? For request-based web-services that means we return an incorrect reply, but hopefully in the future we give correct replies as the faulty servers are dropped. But is it possible, this may corrupt the core state of the application, and lead to returning incorrect replies for further requests?
+ What if we extend our focus from web-services to big data processing systems? Since they are important, they are designed in a fault-tolerant manner, mostly masking fault-tolerant manner: MR, Spark. And who cares if job fails, just restart. But are there examples of very long running cloud systems/daemons, where simple fault-tolerance does not work. The cloud computing fault-tolerance papers may have some examples. Let's see if there is an example?
